Batch Tournament Selection for Genetic Programming

Lexicase selection achieves very good solution quality by introducing ordered test cases. However, the computational complexity of lexicase selection can prohibit its use in many applications. In this paper, we introduce Batch Tournament Selection (BTS), a hybrid of tournament and lexicase selection which is approximately one order of magnitude faster than lexicase selection while achieving a competitive quality of solutions. Tests on a number of regression datasets show that BTS compares well with lexicase selection in terms of mean absolute error while having a speed-up of up to 25 times. Surprisingly, BTS and lexicase selection have almost no difference in both diversity and performance. This reveals that batches and ordered test cases are completely different mechanisms which share the same general principle fostering the specialization of individuals. This work introduces an efficient algorithm that sheds light onto the main principles behind the success of lexicase, potentially opening up a new range of possibilities for algorithms to come.

==> notused.tex <==
\section{On the Survival of Specialists}
\danilo{
The survival of specialists is strongly linked with the success of lexicase.
In fact, in many areas of evolutionary computation, the evolution of specialists have been shown to overcome the problems of generalists.
This happens because creating the solution for the whole problem is harder than breaking the problem into parts and solving each of them.
For example, learning classifier systems \cite{lanzi2000learning},\cite{sigaud2007learning} divide the problem into many condition-action individuals which break the problem and allow each individual to focus on solving a smaller portion of it.
Sometimes, generalists (individuals with conditions that always activate) dominate the population causing a decrease in fitness and diversity.
Self-organizing classifiers \cite{vargas2013self}, \cite{vargas2013aself} goes a step further and create the concept of niched fitness which breaks the fitness into one for each niche, allowing specialists to survive and making generalists only appear when they are as good as specialists. 
Lexicase can also be seen as breaking the fitness function into multiple niched ones.
EDAs had a great success by avoiding mixing different and unrelated variables by joining correlated variables into metavariables \cite{de2014phylogenetic}, \cite{hauschild2011introduction}.
This allowed the evolution of each metavariable independently.
}

\danilo{
Moreover, in \cite{vargas2015general} it was shown that there is a deleterious competition within population. 
In other words, there is no balance between selection pressure and diversity but a competition between the two which causes one to dominate and drive population to easily found solutions.
To avoid this it was shown that complete isolation into subpopulations is key.
Lexicase also isolate specialists to preserve them, i.e., the only way to win against a specialist is to surpass it in its own niche (a certain ordered sequence).
%Dividing the individuals into subpopulations without competition in-between allowed solved the problem.
}

==> related_works.tex <==
Evolution needs selection to bring forth better candidate solutions.
Throughout evolution, these better candidate solutions will help generate even better ones.
This will drive evolution towards candidate solutions with high fitness.
However, the process of generating better candidate solutions needs an important ingredient, diversity.
Populations that lack diversity will consequently fail to explore the fitness landscape.

Selection and diversity are opposing forces in evolution.
And depending on the selection method chosen, a completely different trade-off takes place.
%However, even when diversity is equally preserved, not all selections are the same.
Proportionate reproduction (roulette) is one of the first proposed selection methods.
It is not easy to control selection pressure in it but the time complexity when efficiently coded can achieve $O(n)$ for population of size $n$.

Tournament selection is another widely known method which selects individuals based on tournament winners.
Since weaker individuals have less chance to be chosen in bigger tournaments, the tournament size provides the selection pressure \cite{miller1995genetic}.
Tournament selection is a relatively fast method with time complexity $O(n)$.
It can be easily parallelized and have a selection pressure that can be easily adjusted \cite{goldberg1991comparative}.

Recently, lexicase selection was proposed.
It selects individuals that perform well in random test sequences. 
In this manner, the variance of the sequence distribution provides a good trade-off between diversity and selection pressure \cite{spector2012assessment}.
Interestingly, random test sequences force candidate solutions to solve well small portions of the problem and therefore tends to select candidate solutions which are specialists.
This is in strong contrast with the widespread use of average of solutions which select generalists.
In fact, lexicase have been shown to outperformed other methods in many different scenarios \cite{helmuth2015solving},\cite{helmuth2015general}, \cite{liskowski2015comparison}.
A big disadvantage, however, lies in its time complexity which is $O(n^2)$.

